On the utility of power spectral techniques with feature selection techniques for effective mental task classification in noninvasive BCI

In this paper classification of mental task-root Brain-Computer Interfaces (BCI) is being investigated, as those are a dominant area of investigations in BCI and are of utmost interest as these systems can be augmented life of people having severe disabilities. The BCI model's performance is primarily dependent on the size of the feature vector, which is obtained through multiple channels. In the case of mental task classification, the availability of training samples to features are minimal. Very often, feature selection is used to increase the ratio for the mental task classification by getting rid of irrelevant and superfluous features. This paper proposes an approach to select relevant and non-redundant spectral features for the mental task classification. This can be done by using four very known multivariate feature selection methods viz, Bhattacharya's Distance, Ratio of Scatter Matrices, Linear Regression and Minimum Redundancy & Maximum Relevance. This work also deals with a comparative analysis of multivariate and univariate feature selection for mental task classification. After applying the above-stated method, the findings demonstrate substantial improvements in the performance of the learning model for mental task classification. Moreover, the efficacy of the proposed approach is endorsed by carrying out a robust ranking algorithm and Friedman's statistical test for finding the best combinations and comparing different combinations of power spectral density and feature selection methods.

==> chapters/table6/table11.tex <==
\begin{table*}
\centering
\setlength\extrarowheight{10pt}
\caption{Comparison of classification accuracy for combination of Wavelet method, (without and with) LR feature selection method and ODT\_SVM, for all six Subjects for ten different triplet mental tasks (3 class problem).}
\label{Table_6-1}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
Task & \multicolumn{2}{c|}{Subject 1} & \multicolumn{2}{c|}{Subject 2} & \multicolumn{2}{c|}{Subject 3} & \multicolumn{2}{c|}{Subject 5} & \multicolumn{2}{c|}{Subject 6} & \multicolumn{2}{c|}{Subject 7} \\ \hline
     & Without LR        & With LR       & Without LR        & With LR       & Without LR        & With LR       & Without LR        & With LR       & Without LR        & With LR       & Without LR        & With LR       \\ \hline
BCL  & 0.65       & 0.88          & 0.62       & 0.88          & 0.62       & 0.78          & 0.52       & 0.75          & 0.63       & 0.75          & 0.72       & 0.89          \\ \hline
BCM  & 0.84       & 0.95          & 0.74       & 0.89          & 0.51       & 0.72          & 0.48       & 0.72          & 0.81       & 0.95          & 0.88       & 0.96          \\ \hline
BCR  & 0.77       & 0.93          & 0.82       & 0.98          & 0.52       & 0.69          & 0.57       & 0.76          & 0.76       & 0.88          & 0.90        & 0.95          \\ \hline
BLM  & 0.82       & 0.93          & 0.69       & 0.83          & 0.61       & 0.82          & 0.53       & 0.75          & 0.69       & 0.83          & 0.79       & 0.93          \\ \hline
BLR  & 0.81       & 0.93          & 0.82       & 0.93          & 0.55       & 0.71          & 0.61       & 0.82          & 0.66       & 0.78          & 0.82       & 0.96          \\ \hline
BMR  & 0.93       & 0.99          & 0.77       & 0.93          & 0.52       & 0.67          & 0.63       & 0.79          & 0.76       & 0.86          & 0.77       & 0.94          \\ \hline
CLM  & 0.78       & 0.98          & 0.80        & 0.91          & 0.59       & 0.77          & 0.45       & 0.74          & 0.76       & 0.88          & 0.92       & 1.00             \\ \hline
CLR  & 0.67       & 0.86          & 0.87       & 0.93          & 0.57       & 0.67          & 0.58       & 0.83          & 0.73       & 0.83          & 0.93       & 1.00             \\ \hline
CMR  & 0.85       & 0.94          & 0.84       & 0.96          & 0.43       & 0.66          & 0.59       & 0.78          & 0.8        & 0.9           & 0.82       & 0.95          \\ \hline
LMR  & 0.91       & 0.95          & 0.89       & 0.99          & 0.53       & 0.70           & 0.63       & 0.81          & 0.72       & 0.84          & 0.80        & 0.98          \\ \hline
\end{tabular}
}
\end{table*}

==> chapters/table6/table21.tex <==
\begin{table*}
\centering
\setlength\extrarowheight{10pt}
\caption{Comparison of classification accuracy for combination of Wavelet method, (without and with) LR feature selection method and ODT\_ SVM, for all six Subjects for five different quadruplet mental tasks (4 class problem).}
\label{Table_6-2}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
Tasks & \multicolumn{2}{c|}{Subject 1} & \multicolumn{2}{c|}{Subject 2} & \multicolumn{2}{c|}{Subject 3} & \multicolumn{2}{c|}{Subject 5} & \multicolumn{2}{c|}{Subject 6} & \multicolumn{2}{c|}{Subject 7} \\ \hline
      & Without LR        & with LR       & Without LR        & With LR       & Without LR        & With LR       & Without LR        & With LR       & Without LR        & With LR       & Without LR        & With LR       \\ \hline
BCLM  & 0.70        & 0.84          & 0.62       & 0.77          & 0.48       & 0.71          & 0.40        & 0.64          & 0.63       & 0.77          & 0.73       & 0.87          \\ \hline
BCLR  & 0.62       & 0.85          & 0.66       & 0.87          & 0.47       & 0.66          & 0.48       & 0.68          & 0.59       & 0.73          & 0.72       & 0.88          \\ \hline
BCMR  & 0.73       & 0.91          & 0.71       & 0.91          & 0.39       & 0.60           & 0.48       & 0.69          & 0.68       & 0.83          & 0.72       & 0.88          \\ \hline
BLMR  & 0.81       & 0.92          & 0.70        & 0.85          & 0.44       & 0.65          & 0.51       & 0.68          & 0.58       & 0.73          & 0.66       & 0.88          \\ \hline
CLMR  & 0.71       & 0.84          & 0.74       & 0.91          & 0.44       & 0.62          & 0.44       & 0.71          & 0.65       & 0.79          & 0.76       & 0.96          \\ \hline
\end{tabular}
}
\end{table*}

==> chapters/table6/table31.tex <==
\begin{table*}
\centering
\setlength\extrarowheight{10pt}
\caption{Comparison of classification accuracy for combination of Wavelet method, (without and with) LR feature selection method and ODT\_ SVM, for all six Subjects for a combination of five mental tasks (5 class problem).}
\label{Table_6-3}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
Tasks & \multicolumn{2}{c|}{Subject 1} & \multicolumn{2}{c|}{Subject 2} & \multicolumn{2}{c|}{Subject 3} & \multicolumn{2}{c|}{Subject 5} & \multicolumn{2}{c|}{Subject 6} & \multicolumn{2}{c|}{Subject 7} \\ \hline
      & Without LR         & With LR      & Without LR        & With LR       & Without LR         & With LR      & Without LR         & With LR      & Without LR         & With LR      & Without LR        & With LR       \\ \hline
BCLMR & 0.64       & 0.79        & 0.63       & 0.82         & 0.39       & 0.67        & 0.38       & 0.63        & 0.54       & 0.80        & 0.63       & 0.83         \\ \hline
\end{tabular}
}
\end{table*}

==> chapters/table6/table41.tex <==
\begin{table*}
\centering
\caption{Comparison of the proposed model with existing three methods for three class mental task classification.}
\label{Table_6-4}
\resizebox{\textwidth}{!}{ 
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{10}{|c|}{Three class mental task classification results}                                                                               \\ \hline
     & \multicolumn{2}{l|}{The proposed model} & Li, et al., 2014 & \multicolumn{3}{l|}{Zhang , et al.,2010} & \multicolumn{3}{l|}{Palaniappan, et al., 2002} \\ \hline
Subjects     & Without LR          & With LR        &                  & A           & B            & C           & A1             & B1            & C1            \\ \hline
Subject1 & 0.80        & 0.93          & 0.74             & 0.64        & 0.75         & 0.71        & 0.8            & 0.75          & 0.82          \\ \hline
Subject2 & 0.79        & 0.92          & 0.84             & 0.47        & 0.54         & 0.48        & 0.74           & 0.73          & 0.81          \\ \hline
Subject3 & 0.55        & 0.72           & 0.81             & 0.54        & 0.59         & 0.57        & 0.85           & 0.84          & 0.86          \\ \hline
Subject5 & 0.56        & 0.77          & 0.80              & -           & -            & -           & -              & -             & -             \\ \hline
Subject6 & 0.73        & 0.85          & 0.87             & -           & -            & -           & -              & -             & -             \\ \hline
Subject7 & 0.84        & 0.96          & 0.78             & -           & -            & -           & -              & -             & -             \\ \hline
Average  & 0.71         & \textbf{0.86}          & 0.81            & 0.55        & 0.63        & 0.59       & 0.8            & 0.77          & 0.83          \\ \hline
\end{tabular}
}
\end{table*}

==> chapters/table6/table51.tex <==
\begin{table*}
\centering
\caption{Comparison of the proposed model with existing two methods for four class mental task classification.}
\label{Table_6-5}
\resizebox{\textwidth}{!}{ 
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multicolumn{7}{|c|}{Four Class mental task classification results}                                \\ \hline
      & \multicolumn{2}{l|}{The proposed method} & Li, et al., 2014 & \multicolumn{3}{l|}{Zhang , et al.2010} \\ \hline
Subjects      & Without LR           & With LR       &                  & A           & B           & C           \\ \hline
Suject1  & 0.71         & 0.87         & 0.73             & 0.54        & 0.67        & 0.61        \\ \hline
Suject2  & 0.69         & 0.86         & 0.78             & 0.38        & 0.45        & 0.38        \\ \hline
Suject3  & 0.44         & 0.65         & 0.69             & 0.45        & 0.52        & 0.50         \\ \hline
Suject5  & 0.46         & 0.68         & 0.79             & -           & -           & -           \\ \hline
Suject6  & 0.63         & 0.77         & 0.71             & -           & -           & -           \\ \hline
Suject7  & 0.72         & 0.89         & 0.79             & -           & -           & -           \\ \hline
Average   & 0.61         & \textbf{0.79}         & 0.75            & 0.46       & 0.55       & 0.49       \\ \hline
\end{tabular}
}
\end{table*}

==> chapters/table6/table61.tex <==
\begin{table*}
\centering
\caption{Comparison of the proposed model with existing two methods for five class mental task classification.}
\label{Table_6-6}
\resizebox{\textwidth}{!}{ 
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multicolumn{7}{|c|}{Five class mental task classification results}                                 \\ \hline
      & \multicolumn{2}{l|}{The proposed method} & Li, et al., 2014 & \multicolumn{3}{l|}{Zhang , et al.,2010} \\ \hline
Subjects      & Without LR           & With LR       &                  & A            & B           & C           \\ \hline
Suject1  & 0.64         & \textbf{0.79}         & 0.66             & 0.48         & 0.6         & 0.54        \\ \hline
Suject2  & 0.63          & \textbf{0.82}         & 0.72             & 0.32         & 0.4         & 0.39        \\ \hline
Suject3  & 0.39         & 0.67         &\textbf{0.75}             & 0.39         & 0.46        & 0.44        \\ \hline
Suject5  & 0.38         & 0.63         & \textbf{0.68}             & -            & -           & -           \\ \hline
Suject6  & 0.54         & 0.80         & \textbf{0.85}             & -            & -           & -           \\ \hline
Suject7  & 0.63          & \textbf{0.83}         & 0.75             & -            & -           & -           \\ \hline
Average   & 0.54         & \textbf{0.76}         & 0.74            & 0.39        & 0.49       & 0.46       \\ \hline
\end{tabular}
}
\end{table*}
